Towards Multi-Robot Task-Motion Planning for Navigation in Belief Space

Autonomous robots operating in large knowledgeintensive domains require planning in the discrete (task) space and the continuous (motion) space. In knowledge-intensive domains, on the one hand, robots have to reason at the highestlevel, for example the regions to navigate to or objects to be picked up and their properties; on the other hand, the feasibility of the respective navigation tasks have to be checked at the controller execution level. Moreover, employing multiple robots offer enhanced performance capabilities over a single robot performing the same task. To this end, we present an integrated multi-robot task-motion planning framework for navigation in knowledge-intensive domains. In particular, we consider a distributed multi-robot setting incorporating mutual observations between the robots. The framework is intended for motion planning under motion and sensing uncertainty, which is formally known as belief space planning. The underlying methodology and its limitations are discussed, providing suggestions for improvements and future work. We validate key aspects of our approach in simulation.

==> related_work.tex <==
%Shakey's planner had access to basic geometric knowledge like the objects in a room, and the connectivity between rooms. 

The genesis of TMP can be credited to Fikes and Nilsson for their work on STRIPS~\cite{fikes1971strips} which further led to the Shakey project~\cite{nilsson1984shakey}. Shakey's planner performed a logical search first, assuming that the resulting robot motion plans can be formulated. This assumption limits the capability of the agent as the high-level actions may turn out to be non executable due to geometric limitations. Later works either carried out the generated plans, validating them using a robot motion planner~\cite{dornhege2009SSRR} or performed a combined search in the logical and geometric spaces using a state composed of both the symbolic and geometric paths~\cite{cambon2009IJRR}. The aSyMov planner used in~\cite{cambon2009IJRR} adopts a combination of Metric-FF~\cite{hoffmann2003JAIR} and a sampling based motion planner. In contrast, we use a hybrid temporal task planner~\cite{piotrowski2016AAAI} incorporating robot state uncertainty. Srivastava \textit{et al.}~\cite{srivastava2014ICRA} implicitly incorporate geometric variables, performing symbolic-geometric mapping using a planner-independent interface layer.

%An interface layer then converts PDDL plans to numeric values of the symbols to check the validity of each action in the configuration space. 

%Many of the planning problems need to plan well ahead of time which also results in increased dimensionality, as more and more objects and constraints get added. Longer planning horizons and higher dimensionality directly affects the computational time for these planners. 

Kaelbling and Lozano-P\'{e}res~\cite{kaelbling2012aTR} propose a hierarchical approach that tightly integrates the logical and geometric planning. The complexities arising out of long horizon planning are tackled to the extent that planning is done at different levels of abstraction, thereby reducing the long horizons to a number of feasible sub-plans of shorter horizon. This regression-based planner assumes that the actions are reversible while backtracking. In contrast to their earlier work the serializability assumption of the subgoals is relaxed. This work is extended in~\cite{kaelbling2013IJRR} to consider the current state uncertainty, modeling the planning problem in the belief space. Uncertain outcomes are modeled by converting  a Markov decision processes (MDP) into a weighted graph, thereby modifying their earlier approach of \textit{hierarchical planning in the now}. Belief update is then performed when observations are obtained. Phiquepal and Toussaint~\cite{phiquepal2017RSSws} discuss an ongoing work for TMP under partial observability, computing long-horizon policies that are arborescent in nature. 


The above discussed approaches focus on finding feasible plans sacrificing optimality, emphasizing on performance. Toussaint~\cite{toussaint2015IJCAI} performs optimization over an objective function based on the final geometric configuration (and the cost thereby), finding approximately locally optimal solutions by minimizing the objective function. The planning problem is modeled as a constraint satisfaction problem with symbolic states used to define the constraints in the optimization. Lozano-P\'{e}res and Kaelbling~\cite{lozano2014IROS} model the motion planning as a constraint satisfaction problem over a subset of the configuration space. Iteratively Deepened Task and Motion Planning (IDTMP) is a constraint based task planning approach that incorporates geometric information (motion feasibility) at the task planning level~\cite{dantam2018IJRR}. In our architecture, the waypoints fed into the task planner are generated using the motion planner, similar to the motion planner information that guides the IDTMP task planner. IDTMP performs task-motion interaction using abstraction and refinement functions whereas we use \textit{Semantic attachments}~\cite{dornhege2009ICAPS} to that aim.

FFRob~\cite{garrett2018IJRR} performs task planning by performing search over a sampled finite set of poses, grasps and configurations. In this way, a motion planner is not required as the task planning is performed directly over the sampled set. We also directly perform task planning over a set of sampled poses, implicitly generating motion plans for each task-level actions. PETLON~\cite{lo2018AAMAS} is the work closest to our approach since they also discuss a TMP approach for navigation that is task-level optimal. However, the action costs returned by their motion planner is the trajectory length and they assume completely observable domains. In contrast, we consider a partially observable environment and the costs associated with the uncertainties arising out of the same.
